The Number of Holes in the Union of Translates of a Convex Set in Three Dimensions

We show that the union of $n$ translates of a convex body in $\mathbb{R}^3$ can have $\Theta(n^3)$ holes in the worst case, where a hole in a set $X$ is a connected component of $\mathbb{R}^3 \setminus X$. This refutes a 20-year-old conjecture. As a consequence, we also obtain improved lower bounds on the complexity of motion planning problems and of Voronoi diagrams with convex distance functions.

==> common.tex <==
%%%%%%%%%%%%% define scafolding for front faces (w_i,j)

\path
\foreach \x in {0,...,5}
{ ({50-\x*20}:1) coordinate (w\x) }
;

\path
\foreach \x in {0,...,5}
{
 \foreach \y in {0,...,3}
 {
  (w\x) ++({-.15*\y},0,{1-(.4)^\y}) coordinate (w\x_\y) 
 }
}
;


%%%%%%%%%%%%%%%%%%% define vertices for cuts (v_i,j)

\foreach \y in {0,...,3}
{
 \path (w0_\y) coordinate (a); 
 \foreach \x in {1,...,5}
 {
  \path
  (w\x_\y) coordinate (b)
  ($(a)!{.25*\y}!(b)$) coordinate (v\x_\y)
  (b) coordinate (a);
 }
}


%%%%%%%%%%%%%%% define vertices for the back

\path
\foreach \x in {0,...,5}
{ (0,0,0) ++({50-\x*20}:-1) coordinate (s\x)
  ++(0,0,.936) coordinate (t\x)}
;


